Cut-restriction: from cuts to analytic cuts

Cut-elimination is the bedrock of proof theory with a multitude of applications from computational interpretations to proof analysis. It is also the starting point for important meta-theoretical investigations including decidability, complexity, disjunction property, and interpolation. Unfortunately cut-elimination does not hold for the sequent calculi of most non-classical logics. It is well-known that the key to applications is the subformula property (a typical consequence of cut-elimination) rather than cut-elimination itself. With this in mind we introduce cut-restriction, a procedure to restrict arbitrary cuts to analytic cuts (when elimination is not possible). The algorithm applies to all sequent calculi satisfying language-independent and simple-to-check conditions, and it is obtained by adapting age-old cut-elimination. Our work encompasses existing results in a uniform way, and establishes novel analytic subformula properties.

==> attempt.tex <==

The above proof of the analytic cut property for $\BiInt$ in not tailored to this specific calculus.
In this section we abstract the proof, and introduce sufficient conditions for a sequent calculus to admit restrictions to analytic cuts
As an instantiation of this result, we provide an alternative proof of the analytic cut-property for the calculus in~\cite{OhnMat57} for $\SF$.

\begin{definition}
\label{standcalc}
We call any consistent propositional sequent calculus {\em standard} when it satisfies the following conditions:
\begin{enumerate}
\item axioms have the form $p \seq p$, for $p$ variable
\item the calculus contains all structural rules (weakening, exchange and permutation)
\item each logical/modal rule in the calculus
   \begin{enumerate}
      \item has left and right versions, according to the side of the sequent it modifies;
      \item introduces only one connective/modality at a time;
    \item has no side conditions limiting its application (besides, possibly, a condition saying
           that succedents/antecedents are empty or contain only certain formulas, e.g.
           $\Box$-formulas)
      \item has active formulas that are immediate subformulas of the principal
      formula.
   \end{enumerate}
   \end{enumerate}
\end{definition}

The applicability of cut-restriction in a  (standard) sequent calculus relies on the following properties of the calculus:
its rules allow the replacement of cuts by smaller ones (i.e. logical/modal rules
are {\em reductive}), and for each connectives either both the left and right introduction rules are {\em semi-analytic hp-invertible}, or they allow to perform suitable substitutions. Formally,

\begin{definition}
Let $S$ be any standard sequent calculus. We call its (logical or modal) rules
$\{(\star, r)_1, \dots , (\star, r)_n\}$ and
$\{(\star, l)_1,$ $ \dots , (\star, l)_m\}$ for introducing a connective/modality $\star$
{\em reductive}, if for every instance of the rules
the sequent obtained via (cut) on the principal formula of the conclusions
of $(\star, l)_i$ and $(\star, r)_j$ (for each $i= 1, \dots, m$ and $j=1, \dots m$)
can be derived from their premises using (cut) and the structural rules of $S$.
\end{definition}

We write $\prv{X}{\Gamma\Sa\Delta}$ if the sequent $\Gamma\Sa\Delta$ has a proof of height $\le h$ in which all non-analytic cuts have a cut formula in $X$, and wtite $\psf(A)$ to indicate the set of proper subformulas of $A$. Note that if $A$ is atomic, then $\psf(A)=\emptyset$. 

\begin{definition}
A logical rule with principal formula $F$ and conclusion $S_1$ is \emph{ 
semi-analytic hp-invertible} if whenever $\prv{F} S_1$, then $\prv{F \cup\psf(A)} S_i$ for any premise $S_i$ of that rule.
\end{definition}


The reductivity condition is also one of the key (sufficient) conditions to prove cut-elimination in standard calculi (see, e.g.,~\cite{restall:1999a}); the other being the possibility to shift any cut not on the principal formula upwards. 
For cut-restriction we need to relax this second condition, making use of the following notion.

\begin{definition}
Let $S$ be any standard sequent calculus. A rule 
$$\small
\infer[(r)]{\Gamma \seq \Delta}{\Gamma_1 \seq \Delta_1  \dots  & \dots 
 \Gamma_n \seq \Delta_n}$$
is said to be {\em  L-replaceable} (resp. R-replaceable) with a sequent $\Gamma' \seq \Delta'$ if
 for every instance of the rule and any occurrence of the formula $X$, which is not
the principal formula of $(r)$, by cutting possibly multiple times
its conclusion with $\Gamma', X \seq \Delta'$ (resp. $\Gamma' \seq X, \Delta'$) and all corresponding $X$' in its premises (w.r.t. the predecessor relation)
results in a correct application of the rule (possibly using the structural rules).
\end{definition}





\begin{theorem}
In any standard sequent calculus $S$, safisfying the following conditions: 
For every connective/modality $\star(A_1 \dots A_n)$
\begin{enumerate}
    \item its rules are reductive
 \item either its left and right introduction rules are semi-analytic hp-invertible, or they satisfy either for the left or
\begin{itemize}
\item[2.(i)] the left rule (or resp. right) rule introducing $\star(A_1 \dots A_n)$ can be transformed into an axiom by replacing the principal formula  $\star(A_1 \dots A_n)$ with a multiset of formulas (not containing $\top$ or $\bot$)
\item[2.(ii)] every rule is R-replaceble (or resp. L-replaceble) with
the context of the left rule (resp. right) rule introducing $\star(A_1 \dots A_n)$
\item[2.(iii)] all the other calculus rules are L-replaceable  (or resp. L-replaceble)        with the multiset of formulas in 2.(i).
\end{itemize}
\end{enumerate}
cut-restriction holds.
\end{theorem}
\begin{proof}
Let $\delta$ be a proof ending in a non-analytic cut 
\[
\infer[\cut]{\Gamma\Sa \Delta}
	{
	\infer*[\delta_L]{\Gamma\Sa C,\Delta}{}
	&
	\infer*[\delta_R]{\Gamma, C\Sa \Delta}{}
	}
\]
and assume that the subproofs $\delta_L,\delta_R$ are locally analytic. We distinguish cases according to the shape of $C$.
\begin{itemize}
\item The case $C$ is atomic, follows the same pattern as in the proof of $\BiInt$, being
the calculus standard.
\item Let $C$ be a compound formula with most external connective
$\star'(A_1 \dots A_n)$ whose left and right rules are semi-analytic hp-invertible. By using this property, together with reductivity we get a proof of the same end-sequent having only non analytic cuts on $\psf(A_1), \dots ,\psf(A_n)$ which then can be handled by the inductive hypothesis. 
\item Assume now that $C= \star(A_1 \dots A_n)$ and either one of the left or of the right (or both) introduction rules for $\star(A_1 \dots A_n)$ is not semi-analytic hp-invertible. We follow the pattern in the proof for $\BiInt$ of $\impl$. W.l.o.g. we can assume that the proof is irredundant (this property is guaranteed by the presence of contraction). We trace the predecessors of the cut formulas in $\delta_L$ and $\delta_R$. 
Step 1 in the proof goes through using reductivity of the rules and the inductive hypothesis
(on the smaller non-analytic cuts). Step 2 follows by property 2.(i) and 2.(iii). Step 3 follows by property 2.(ii).
\end{itemize}
\end{proof}


==> attempt2.tex <==

\agata{DISCLAIMER: We need to formalize the notion of sequent calculi we work with: let us call them \emph{standard sequent calculi}
\begin{itemize}
    \item needed properties: consistent, atomic identity axioms, all structural rules, rules expressed as rule schemas (we can take inspiration by Ori Lahav's papers)
\end{itemize}
}

The following three properties are well known to proof theorists:

\begin{enumerate}
    \item[(AC1)] \textbf{principal reductions:} replace a cut that is principal in left and right premise by cuts on smaller formulas
    (see Sect.~\ref{sec-idea}).
    
    \item[(AC2)] \textbf{invertibility} of rules: given a proof of the conclusion of a logical rule there are proofs of its premises with no new cuts.
\marginpar{I am not considering constants for the time being}    
  \item[(AC3)] \textbf{axiom expansion:} completeness of atomic axioms.  
\end{enumerate}
When these properties hold for all connectives of a standard sequent calculus cuts can be reduced to smaller cuts. Indeed any cut on a compound formula $C$ can be transformed into cuts on smaller cut-formulas by replacing $C$ with its immediate subformulas by invertibility and apply the principal cut reduction. 

For cut-elimination we still need to remove atomic cuts; if the rules of the considered calculus are all L-substitutive or all R-substitutive the task can be accomplished, where:
\begin{itemize}
    \item \textbf{L-substitutivity} (resp. \textbf{R-substitutivity}): every cut with cut-formula on the LHS (resp. RHS) which is not principal can be shifted upwards.
\end{itemize}
Actually, if the calculus rules are both L \emph{and} R-substitutive, rules invertibility is not needed to prove cut-elimination and Genten's standard procedure applies. Even when some of these conditions fail, cut-elimination might still be possible.

\begin{example}
\label{ex:Mae}
This is the case of Maehara's propositional calculus~\cite{Takeuti:87} for IL -- a multiple-conclusion sequent calculus in which \textit{the succedent of the ${\imp}_R$ rule permits no context}, 
\[
\infer[\imp_L]{\Gamma,A\imp B\Sa\Delta}
	{
	\Gamma\Sa A,\Delta
	&
	\Gamma, B\Sa\Delta
	}
\hspace{2cm}
\infer[\imp_R]{\Gamma\Sa A\imp B}
	{
	\Gamma,A\Sa B
	}
\]
Although the calculus admits cut-elimination, the rule $\imp_R$ is not invertible and (due again to this rule) the calculus rules are not L-substitutive.
\end{example}

We relax the above conditions. Indeed, cut-elimination also holds when \emph{all} the calculus rules are R-substitutive (resp. L-substitutive) \emph{and} for each non-invertible connective $\circ$ a restricted form of substitutivity holds: we only require to shift upwards cuts with cut-formula on the LHS (resp. RHS), whose other premise is the conclusion of a rule introducing $\circ$ on the RHS (resp. LHS). Namely, we require that each non-invertible connective $\circ$ is $\circ$-L-substititive (resp. $\circ$-R-substititive).

\begin{itemize}
    \item[(AC4)] \textbf{$\circ$-L-substititive}
    (resp. \textbf{$\circ$-R-substititive}) ....
\end{itemize}

It is easy to see that cut-elimination holds for sequent calculi in which conditions (AC1), (AC3), R-substitutivity (respectively L-substitutivity) hold, and for each connective $\circ$, either $\circ$ is invertible both on the RHS and on the LHS, or it is $\circ$-L-substitive (resp. $\circ$-R-substitutive).

\begin{example}
The above conditions (and the corresponding cut-elimination strategy) work for Maehara's calculus for IL but they do not for the sequent calculus $\BiInt$~\cite{Rau74} for bi-intuitionistic logic. $\BiInt$ is 
obtained from the Maehara calculus by extending the language with \textit{coimplication}~$\coimp$ and adding the following rules 
\[
\infer[\coimp_L]{A\coimp B\Sa\Delta}
	{
	A\Sa B,\Delta
	}
\hspace{2cm}
\infer[\coimp_R]{\Gamma\Sa A\coimp B,\Delta}
	{
	\Gamma\Sa A,\Delta
	&
	\Gamma,B\Sa \Delta
	}
	\]
This is not a suprise,  as	$\BiInt$ does not admit cut-elimination.
In this calculus indeed the right rule of $\imp$ and the left rule of $\coimp$ are not invertible and the calculus rules are neither L-substitutive (due to $\imp_R$) nor R-substitutive (due to $\coimp_L$). $\BiInt$ is howevr complete when restricted to analytic cuts
\end{example}
We formulate below general conditions that guarantee that given a proof with cut it can be transformed into a proof only containing analytic cuts (cut-restriction). First of all notice that in the context of keeping analytic cuts we do not care anymore about removing atomic cuts, hence the condition that all the calculus rules have to be either L-substitutive or R-substitutive can be dropped.
To prove cut-restriction a form of regularity is needed to deal with non invertible connectives $\circ$ who are $\circ$-R-substitutive (resp. $\circ$-L-substitutive), namely that they are also $\circ$-R-regular (resp. $\circ$-L-regular).
To fix ideas, let $X \seq \circ (A_1, \dots , A_n), Y$ be a (n instance of the) conclusion of a rule introducing $\circ$ on the RHS (resp. $X', \circ(A_1, \dots, A_n) \seq Y'$ on the LHS):
\marginpar{If we enforce the isolation of the introduced formula the main proof if simpler}

\begin{enumerate}
  \setcounter{enumi}{3}
    \item[(AC5)]
    \textbf{$\circ$-R-regular:} 
    (resp. \textbf{$\circ$-L-regular:})
%For every rule instance $r$ the replacement of any congruent\footnote{I am using a terminology from display calculus} context formula on the RHS and on the LHS with possibly many formulas from $X$ and Y (resp. from $X'$ and $Y'$) still results in a rule instance.
\end{enumerate}


\begin{example}
In the calculus $\BiInt$ $\imp$ is L-substitutive and R-regular and $\coimp$ is R-substitutive and L-regular.
\end{example}




==> figure1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Triangle [id:dp21331741976996332] 
\draw   (163,121) -- (85,54) -- (241,54) -- cycle ;
%Shape: Triangle [id:dp5610904427388644] 
\draw   (350,123) -- (272,56) -- (428,56) -- cycle ;
%Shape: Triangle [id:dp4105093499075788] 
\draw   (372.5,227) -- (147,154) -- (598,154) -- cycle ;

% Text Node
\draw (79,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma _{1} ,\Delta _{1}$};
% Text Node
\draw (142,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma _{2} ,\Delta _{1}$};
% Text Node
\draw (214,31) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (143,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \gamma [ \Delta _{1}]$};
% Text Node
\draw (266,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma _{1} ,\Delta _{2}$};
% Text Node
\draw (329,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma _{2} ,\Delta _{2}$};
% Text Node
\draw (401,33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (330,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \gamma [ \Delta _{2}]$};
% Text Node
\draw (446,119) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (145,125) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma ,\Delta _{1}$};
% Text Node
\draw (332,126) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma ,\Delta _{2}$};
% Text Node
\draw (354,178) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \delta [ \Gamma ]$};
% Text Node
\draw (354,233) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Gamma ,\Delta $};


\end{tikzpicture}


==> intro.tex <==
%%NEW VERSION REV 12 JAN%%


The fundamental result in proof theory is cut-elimination. It is the syntactic algorithm that eliminates cuts from a sequent calculus proof leading to an analytic proof, i.e., only containing formulas which are subformulas of the final statement.
%Cut-elimination applies to many logics irrespective of their semantics.
Though larger in size, analytic proofs are much better behaved and more amenable to meta-theoretic investigation, as the space of proofs under consideration is greatly constrained. 
%As Smullyan~\cite{Smu68} observes, ‘the real importance of cut-free proofs is not the elimination of cuts per se, but rather that such proofs obey the subformula principle’. 
Gentzen's motivation in the 1930's was a relative consistency of arithmetic but the influence of cut-elimination is far beyond that. 
From its interpretation as computation under the proofs-as-programs correspondence (e.g.~\cite{CH06}) 
%NOT RELEVANT that extends to concurrency (linear logic and the $\pi$-calculus), 
to its role in proof analysis  (e.g.~\cite{BaazHLRS08}), 
% ELEMENTARY PROOFS HAVE NO for obtaining elementary proofs~\cite{BaazHLRS08}, 
it is by far the most fundamental proof transformation.
Moreover, cut-free calculi --that are the offspring of cut-elimination-- are used to prove metalogical properties of the underlying logics (e.g., decidability, upper bounds, various flavours of interpolation, and disjunction properties), and key to develop automated reasoning methods. 

Given the influence of Gentzen's seminal result it was inevitable that it would be extended to more and more logics.
Cut-elimination was originally proved for the sequent calculi for classical and intuitionistic logic IL but from that time onwards right up to the present day, new interesting and useful logics continue to be introduced and so the program of developing cut-free calculi via cut-elimination was extended. The first significant obstacle was encountered in the early 1950's: how to eliminate cuts in the proof calculus for the modal logic $\SF$? 
%While syntactic decision arguments for $\SF$ were obtained (see Ohnishi and Matsumoto~\cite{OhnMat57,OhnMat59}), it seems that 
In 1968, Mints~\cite{Min68} solved the problem but not using the sequent calculus. He instead proved cut-elimination for $\SF$ using a generalisation of the sequent calculus known today as the hypersequent calculus, e.g.~\cite{Avr96}. This ushered in era of frenetic activity in proof theory: generalising the sequent calculus to obtain a proof calculus where the cut-rule is eliminable for the various  logics of interest. Numerous generalising proof formalisms have been introduced in the intervening period: nested, labelled, bunched, tree-hypersequent, display sequent calculi, and many more.

And yet it is the sequent calculus rather than any of these other formalisms that remains familiar to anyone with a passing knowledge of formal logic. Aside from its association with Gentzen's famous result, reasons include its simplicity, the ready identifiability of a sequent with logical consequence (the set of assumptions is on the left of the sequent and consequences appear on the right),  and the numerous meta-logical results that have been proved using it. 

Given the great attraction of the sequent calculus and faced with the reality that cuts cannot be always eliminated, %from calculi
%we cannot always eliminate cuts from the sequent calculus of some logic 
we are led to an alternative approach: retain the sequent calculus and identify the ``minimal" cuts that are required for completeness. 
Staying with the sequent calculus means retaining the clear interpretation between sequent and formula, a single target for automated theorem proving, proof-assistants, and meta-theoretic argumentation. In brief, a single target for theory and applications.


The most natural cuts to accept are \textit{analytic cuts} i.e. the cut-formula is a subformula of the input formulas. This directly leads to the subformula property~\cite{KowOno17}, and as Smullyan~\cite{Smu68} observes, ‘the real importance of cut-free proofs is not the elimination of cuts per se, but rather that such proofs obey the subformula principle’.
Indeed decidability, complexity and interpolation arguments seem to hold in the presence of analytic cuts, e.g.,~\cite{??,Tak92,OnoSano}. For instance,
Kowalski and Ono~\cite{KowOno17} show a host of results utilising analytic cut property such as Craig interpolation, Halld\'{e}n completeness and Maximova variable separation.
Apart from this, the usual blow-up in the size of cut-free proofs can be alleviated if one admits analytic cuts~\cite{dAgo92} (deterministic speed-up).

Semantic methods have been used to show that  
%There are several results using semantics to show that 
a restriction to analytic cuts suffices for completeness (see e.g.~\cite{Fit78,DAgoMon94,KowOno17,AvrLahav}),
%(in some cases, slight modifications of the subformula property), 
In some cases~\cite{Tak01,Tak19,Tak20} slight modifications of the property have also been investigated. 
%Furthermore, Kowalski and Ono~\cite{KowOno17} show a host of results utilising analytic cut property such as Craig interpolation, Halld\'{e}n completeness and Maximova variable separation.
%
%However 
%the analytic cut property 
However, these methods \textit{lack} two important features of Gentzen's cut-elimination argument: applicability across diverse proof systems irrespective of the logic's semantics, and an algorithm to eliminate cuts from a proof in a stepwise manner. Indeed, the constructive nature of cut-elimination was important to satisfy Hilbert's requirement for a finitistic proof of consistency. Even beyond this, it is crucial for proof analysis, ordinal analysis, proof complexity, and computational interpretations. 
Therefore we seek a general and constructive methodology and we call this \textit{cut-restriction}. 

Cut-elimination is then a special, boundary case of cut-restriction. It sufficed for Gentzen's original aims
%---a relative consistency proof of arithmetic---
but it is too stringent for the many logics that we wish to study. In 1992, Takano~\cite{Tak92} took up the challenge to obtain cut-restriction up to analytic cuts (in our terminology) for $\SF$. 
This result is well-known but the method itself seems to be largely unknown, possibly due to the intricate arguments that are involved. 
A different approach for $\SF$ appears in Ciabattoni \textit{et al.}~\cite{CiaLanRam21} where,  starting with a cut-free hypersequent calculus, the hypersequent structure is systematically removed in favour of analytic cuts. This extends to large classes of substructural, intermediate, and modal logics (the cuts are not necessarily analytic any more but they are still controlled by the input in a precise sense). %The work~\cite{CiaLanRam21} is an excellent proof-of-principle but 
%it relies on the existence of cut-free hypersequent calculi
%us and its cut-elimination so it cannot be considered as an alternative to generalised proof formalisms. 
%Moreover, 
The method can only be applied starting with cut-free hypersequent calculi, the complex sequence of transformations in no way resembles Gentzen's reductions, and they do not witness cut-elimination as a special case of cut-restriction. Nevertheless \cite{CiaLanRam21} provides an excellent proof-of-principle for cut-restriction.
%(so it is not an alternative to generalised proof formalisms)}.
%NOTE that cut elimination for those logics DOES NOT hold}
% NOOOOOOO, see our LICS and TCS papers and they obscure a computational interpretation.}
%
%This is the starting point for this work. 
Armed with that knowledge that cut-restriction is possible, we show how to extend Gentzen's cut-elimination to obtain a constructive argument for cut-restriction. 
We introduce an algorithmic transformation of proofs with arbitrary cuts into proofs with analytic cuts.
Our proof is formulated using language-independent conditions along the line of Belnap's~\cite{Bel82} general conditions for cut-elimination, and apply to sequent calculi having all structural rules and whose logical rules introduce one connective at a time.

Not only do we identify sufficient conditions for cut-restriction, 
%we reveal underlying principles sufficient for getting analytic cuts
%(yielding a simplified argument for $\SF$ w.r.t.~\cite{Tak92}), 
it is now evident that cut-elimination is a special case. 
Our work brings together scattered results in the literature, provides a uniform way to prove
the analytic cut-property for a host of calculi (in particular, simplifying Takano's argument for $\SF$),
and resolving the following open question for bi-intuitionistic logic which is a conservative extension of IL:
\begin{itemize}
\item The calculus $\BiInt$ of~\cite{Rau74}: Semantic proofs were presented independently by Kowalski and Ono~\cite{KowOno17}, and Avron and Lahav~\cite{AvrLahav}. \cite{PintoU18} proved syntactically that infinitely many cut-formulas of a certain (co)implicational form suffice for completeness but left open the problem of finding a constructive procedure for the analytic cut property.
%but a constructive procedure was left open in~\cite{PintoU18}, where it was shown that infinitely many formulas of a certain (co)implicational form ensure completeness.
%\item $L_4$~\cite{Ono77}: even analytic cut property was open (\cite{OnoSano}).
\end{itemize}
Further calculi that satisfy our conditions and were not known before to have the analytic
cut property include the calculus {\bf L4} in~\cite{Ono77} for the strongest S5-type intuitionistic modal logic {\bf G4}, and its extension with the coimplication connective. 

%Our work encompasses various existing results, and allows for the discovery of the analytic cut-property for existing calculi and new logics.

%Moreover checking the conditions for new logics is straightforward. 
%\begin{itemize}
%\item bi-intuitionistic logic: the cut-restriction problem was left open in~\cite{PintoU18}. Semantic proofs were presented independently by Kowalski and Ono~\cite{KowOno17}, and Avron and Lahav~\cite{AvrLahav};
%
%\item $L_4$~\cite{Ono77}: even analytic cut property was open. Moreover, we identify the general reductions that are required (yielding a much simplified argument for cut-restriction of $\SF$), and cut-elimination is obtained as a special case. 
%\end{itemize}
 
 

\smallskip
\subsubsection*{Cut-restriction needs a novel idea}

It might seem reasonable to assume that cut restriction follows from some slight amendment of cut-elimination.
We illustrate using the case of $\SF$ that this is \textit{not} the case.
%We are confident that Takano's analytic cut property result for $\SF$ is known to every proof theorist. It would seem reasonable to assume that the result follows from some slight amendment of cut-elimination but this is \textit{not} the case. Indeed, let us see 
%why cut-elimination does not help with cut-restriction. 
The following presumes some knowledge of cut-elimination; the reader unfamiliar with this terminology is referred to the section that follows. Consider the cut below that is well-known to be not eliminable in $\SF$ (see e.g. Ono~\ref{Ono19book}).
\begin{center}
\AxiomC{$\Box\lnot p\Ra \Box\lnot p$}
\UnaryInfC{$\Ra \lnot\Box\lnot p,\Box\lnot p$}
\RightLabel{5}
\UnaryInfC{$\Ra \Box\lnot\Box\lnot p,\Box\lnot p$}
%
\AxiomC{$p\Ra p$}
\UnaryInfC{$\lnot p,p\Ra$}
\RightLabel{T}
\UnaryInfC{$\Box\lnot p,p\Ra$}
%
\RightLabel{cut}
\BinaryInfC{$p\Ra \Box\lnot\Box\lnot p$}
\DisplayProof
\end{center}
%The cut-formula is principal in both premises of the cut NO. It is NOT principal in the left premise
Observe that the the cut-formula is principal in the right premise by (T) and it is non-principal in the left premise by (5).
Therefore the usual move in cut-elimination would be to lift the cut upward in the left premise which means a cut on
$\Ra \lnot\Box\lnot p,\Box\lnot p$ and $\Box\lnot p,p\Ra$ yielding $p \Ra \lnot\Box\lnot p$. However there is no way to proceed from the latter; in particular we cannot apply ($5$) as that rule requires that every context formula is boxed.\footnote{The non-existence of a cut-free proof of $p\Ra \Box\lnot\Box\lnot p$ can be shown by exhaustive consideration of potential proofs rooted at this sequent.} %but being
%analytic ($\Box\lnot p$ is a subformula of $p\Ra \Box\lnot\Box\lnot p$) }
%, as we cannot reach a situation in which the cut-formula is principal in both premises to apply a principal-reduction and obtain a smaller cut.}
%
Note that the cut in the proof diagram is analytic because $\Box\lnot p$ is a subformula of $p\Ra \Box\lnot\Box\lnot p$. So if we are prepared to accept analytic cuts then 
nothing more needs to be done here. Of course, it still remains to show that analytic cuts suffice in all situations. Since we seek a constructive proof, the natural idea would be to generalise cut-elimination by considering an arbitrary topmost non-analytic cut and aiming reductions to make the cut-formula smaller until the cut disappears or
becomes analytic. But how to proceed with the following cut?
%Now consider the following cut on an arbitrary formula~$\Box A$.
\begin{center}
\AxiomC{$\Box\Gamma\Ra \Box A, B $}
\RightLabel{5}
\UnaryInfC{$\Box\Gamma\Ra\Box A,\Box B$}
%
\AxiomC{$A,\Sigma\Ra\Pi$}
\RightLabel{T}
\UnaryInfC{$\Box A,\Sigma\Ra\Pi$}
%
\RightLabel{non analytic cut}
\BinaryInfC{$\Box\Gamma,\Sigma\Ra\Box B,\Pi$}
\DisplayProof
\end{center}
Just as in the example above, the cut-formula is principal in the right premise by (T) and non-principal in the left premise by (5). 
We have already noted that this situation is problematic so 
a new idea is needed in order to proceed. Even the briefest consideration of~\cite{Tak92} will provide an indication of the intricacy of Takano's solution.

\medskip
\agata{The paper is organized as follows. The idea behind cut-restriction is discussed informally in Section~\ref{sec-idea} using $\BiInt$ as case study. The main ingredients for the cut-restriction proof to go through are identified in Section~\ref{sec:SC}; they are formulated in terms of syntactic sufficient conditions to be satisfied by a sequent calculus with all structural rules and whose logical/modal rules introduce one connective at a time ({\em standard sequent calculus}). The main proof is .... bla}

%%NEW VERSION END%%

% Cut-elimination is the bedrock of  proof theory. It is the syntactic algorithm that eliminates cuts from a sequent calculus proof leading to an analytic proof, i.e., only containing formulas which are subformulas of the final statement.
% %Cut-elimination applies to many logics irrespective of their semantics.
% Though larger in size, analytic proofs are better behaved and more amenable to meta-theoretic investigation, as the space of proofs under consideration is greatly constrained. Gentzen's motivation in the 1930's was a finitistic proof of the consistency of arithmetic (paving the way for ordinal analysis) but the influence of cut-elimination is far beyond that. The cut-free calculi that are the offspring of cut-elimination are used to prove metalogical properties of the underlying logic (e.g., consistency, decidability, upper bounds, various flavours of interpolation, and disjunction properties), and key to develop automated reasoning methods. 

% Let us pick up the story in the decades following Gentzen's seminal result.
% Cut-elimination was originally proved for the sequent calculi for classical and intuitionistic logic IL. 
% The programme of developing cut-free calculi via cut-elimination was soon extended to more logics, notably modal logics. The first significant obstacle was encountered in the early 1950's: how to eliminate cuts in the proof calculus for the modal logic $\SF$? 
% While syntactic decision arguments for $\SF$ were obtained (see Ohnishi and Matsumoto~\cite{OhnMat57,OhnMat59}), it seems that 
% the first proof of cut-elimination was by Mints~\cite{Min68} who extended the metalanguage of %the proof calculus from 
% Gentzen's sequent calculus to essentially what is today called the hypersequent calculus. Hypersequent calculi were rediscovered independently in the 1980's, by Pottinger~\cite{Pot83} to obtain cut-elimination for modal logics, and Avron~\cite{Avr87,Avr96}, who applied them to relevant, modal, and intermediate logics. The floodgates had been opened: when cut-elimination cannot be obtained for a logic of interest, the standard response in structural proof theory is to look for (or invent) a new proof formalism by extending the metalanguage of the sequent calculus such that cut-elimination \textit{does} hold. Most proof formalisms have been introduced in the last three decades in this way; nested, labelled, bunched, linear, tree-hypersequent, display sequent, and many more.

% A question that has instead received little attention in all this time is whether it is possible to adapt cut-elimination to transform those cuts that are not eliminable into `analytic´ cuts, i.e., cuts restricted to subformulas of the conclusion.
% Indeed, as remarked in~\cite{Smu68}, ‘the real importance of cut-free proofs is not
% the elimination of cuts per se, but rather that such proofs obey the subformula principle’. The
% latter does not require the {\em elimination} of cuts. It is sufficient to {\em restrict} applications
% of the cut rule to analytic cuts. This is the subject of the paper.
% %In addition, analytic cuts may also be useful from a computational viewpoint~\cite{DAgoMon94}, and the usual blow-up in the size of cut-free proofs can be alleviated if one admits analytic cuts~\cite{dAgo92}., and the usual blow-up in the size of cut-free proofs can be alleviated if one admits analytic cuts~\cite{dAgo92}.
% %
% %A question that has received little attention in all this time is whether it is possible to adapt  cut-elimination to transform those cuts that are not eliminable into analytic cuts, i.e., cuts restricted to subformulas of the conclusion.
% %
% %The restriction to analytic cuts is of particular conceptual interest because it corresponds directly to the subformula property~\cite{KowOno17}, whereas cut-elimination is a strictly stronger property.
% %
% We introduce cut-restriction -- an algorithmic
% transformations of proofs with arbitrary cuts into proofs with analytic cuts.
% Obtained as an adaptation of age-old cut-elimination,  in cut-restriction 
% Gentzen's permutation reductions are intuitively replaced by intermediary cuts
% %This algorithmic restriction -- which we call cut-restriction -- is the subject of the present paper.
% %We indeed introduce an algorithm to transform proofs from arbitrary cuts to analytic cuts. 
% A result in the spirit of cut-restriction is contained in Takano's 1992 paper~\cite{Tak92} on the analytic cut property for $\SF$. 
% Even there, the argument does not appear to have the generic character that is a hallmark of Gentzen's arguments. Other results restricting cuts rely on the semantics of the logics under consideration, e.g., \cite{Fit78,DAgoMon94,KowOno17,AvrLahav,Tak01,Tak20}.
% In contrast, Gentzen's cut-elimination method applies rather uniformly across diverse proof systems irrespective of the logic's semantics. A major motivation for choosing to adapt cut-elimination as the path to restricting cuts is the ambition that it too will be applicable as broadly. As this regards, our proof of cut restriction is formulated in a general way and applies to sequent calculi satisfying suitable syntactic conditions.
% %formulate sufficient conditions for a sequent calculus to admit cut-restriction. 
% Inspired by Belnap's conditions for cut-elimination in display calculus~\cite{Bel82},
%  our conditions are however not modular, as they have to be checked for all the calculus' rules. This is no surprise, being the analytic cut property not modular either. A main example of a calculus which does not admit cut-elimination but it admits the analytic cut property is the sequent calculus $\BiInt$~\cite{Rau74} for bi-intuitionistic logic, also known as Heyting–Brouwer logic or subtractive logic,  -- a conservative extension of intuitionistic logic with a $\coimp$ connective that is dual to implication ({\em coimplication}).
%  $\BiInt$ contains the connectives $\to$ and $\coimp$ that separately admits cut-elimination, but whose combination does not.
% The analytic cut property for $\BiInt$  was independently proved using semantics in Kowalski and Ono~\cite{KowOno17} and Avron and Lahav~\cite{AvrLahav}. The former paper also exploits it to prove interpolation for bi-intuitionistic logic. The problem of establishing this result using proof-theoretic method was instead left open in~\cite{PintoU18} where it was shown that infinitely many cut-formulas of a certain (co)implicational form ensures completeness. 

% Our sufficient conditions apply to a variety of propositional calculi. Among them,
% to the calculus for $\SF$ and $\BiInt$, already known to have the analytic cut property, as well as to other calculi for which this result was not known before, including the calculus {\bf L4} in~\cite{Ono77} for the strongest S5-type intuitionistic modal logic (its analyticity status was stated in~\cite{OnoSano} as an open problem), and
% the extension of {\bf L4} with the coimplication connective.
% ...Interpolation????
% %In addition to the theoretical interest in adapting this most fundamental notion in proof theory, there are several further motivations.
% %
% %Cut-restriction is an alternative to moving to proof formalisms more complex than the sequent calculus to obtain cut-elimination. New proof formalisms are designed so that the cut-elimination proof goes through, but it is always possible that the same could have been achieved using a simpler formalism.
% %For example, the hypersequent calculus for $S5$\cite{Avr96,Min68} manipulates arbitrarily many component sequents although it turns out that only two are in fact required~\cite{Ind19}. 
% %Additional structure in the proof formalism is often a hindrance to proving metalogical results, and for limiting the proof search space. On the other hand 
% %decidability and complexity arguments proceed in the presence of finitely many sequent cuts, and interpolation proofs too, at least in the case of analytic cuts, e.g.,~\cite{Tak92,KowOno17,OnoSano}.
% %In addition, analytic cuts may also be useful from a computational viewpoint~\cite{DAgoMon94}, and the usual blow-up in the size of cut-free proofs can be alleviated if one admits analytic cuts~\cite{dAgo92}.  

% ...PLAN to be decided ....
% The idea behind cut-restriction is first discussed informally in Section~\ref{sec-idea}, using $\BiInt$ as case study. The main ingredients for the cut-restriction proof to go through are identified in Section~\ref{sec:SC}; they are formulated in terms of syntactic sufficient conditions to be satisfied by a sequent calculus with all structural rules and whose logical/modal rules introduce one connective at a time ({\em standard sequent calculus}). The main proof is in .... INTERPOLATION ....

% %The point in this paper is that  we uncover how to obtain these results as an adaptation of age-old cut-elimination. 
% %


==> k5.tex <==
\section{$K5$ incomplete}

The sequent calculus for $K5$ extends the sequent calculus $LK$ for classical propositional logic with the following rule:
\begin{center}
\AxiomC{$\Gamma\Ra \Box\Theta, A$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma\Ra \Box\Theta, \Box A$}
\DisplayProof
\end{center}
The $5$ axiom is $\lnot\Box p\imp \Box\lnot\Box p$.

Takano (A Modified Subformula Property for the Modal Logics K5 and K5D) shows that every provable sequent has a proof built from formulas that are $K5$-subformulas of the endsequent i.e. subformulas of the endsequent, or $\Box\lnot\Box B$ or $\lnot\Box B$ such that $\Box B$ is an internal subformula (i.e. itself nested under a $\Box$) of the endsequent.

The critical case is the following. As always, we first identify the predecessors of the cut-formulas. For simplicity we suppose a single critical inference in each premise.
\begin{center}
\AxiomC{$\Gamma'\Ra \Box\Theta',A$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma'\Ra \Box\Theta',\Box A$}
\noLine
\UnaryInfC{$\leftpremise$}
\noLine
\UnaryInfC{$\Gamma\Ra \Theta, \Box A$}
%
\AxiomC{$A, X'\Ra \Box Y', B$}
\RightLabel{$5$}
\UnaryInfC{$\Box A, \Box X'\Ra \Box Y', \Box B$}
\noLine
\UnaryInfC{$\rightpremise$ no $5$ rule}
\noLine
\UnaryInfC{$\Box A, X\Ra Y$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, X\Ra \Theta, Y$}
\DisplayProof
\end{center}
We proceed as follows.
\begin{center}
\begin{footnotesize}
\AxiomC{$\Gamma\Ra\Theta,\lnot\Box\Theta'$}
%
\AxiomC{}
\UnaryInfC{$\lnot\Box\Theta'\Ra\Box\lnot\Box\Theta'$}
%
\AxiomC{$\Gamma\Ra\Theta,\Box\Gamma'$}
%
\AxiomC{$\Gamma'\Ra \Box\Theta',A$}
\AxiomC{$A, X'\Ra \Box Y', B$}
\RightLabel{cut}
\BinaryInfC{$\Gamma', X'\Ra \Box\Theta', \Box Y', B$}
\RightLabel{$\lnot R$}
\UnaryInfC{$\Gamma', X', \lnot\Box\Theta'\Ra  \Box Y', \Box B$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma', \Box X', \Box\lnot\Box\Theta'\Ra  \Box Y', \Box B$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X', \Box\lnot\Box\Theta'\Ra  \Box Y', \Box B$}
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X', \lnot\Box\Theta'\Ra  \Box Y', \Box B$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X'\Ra  \Box Y', \Box B$}
\noLine
\UnaryInfC{$+\rightpremise$}
\noLine
\UnaryInfC{$\Gamma, X\Ra  \Box Y$}
\DisplayProof
\end{footnotesize}
\end{center}
It's not enough to choose a topmost cut that is not a $K5$-subformula. We also need that $\Box\Theta'$ is an (internal) subformula of the endsequent, since the above transformation cuts on $\Box\lnot\Box\Theta'$ and $\lnot\Box\Theta'$.

If we can restrict antecedent formulas to subformulas, or $\lnot\Box B$ ($\Box B$ is a subformula), or $\Box\lnot\Box B$ at an initial sequent ($\Box B$ is a subformula) then we might be fine, but I'm not sure how we can do this.



==> s5.tex <==



A sequent calculus $\SF$~\cite{OhnMat57} for the modal logic $S5$ extends Gentzen's calculus $\LK$ for classical propositional logic with the following two rules for the modality~$\Box$:
\begin{equation}\label{SFrules}
\infer[T]{\Gamma,\Box A\Sa\Delta}
    {
    \Gamma,A,\Sa\Delta
    }
\qquad\qquad\qquad
\infer[5]{\Box\Gamma\Sa\Box A,\Box\Theta}     {
    \Box\Gamma\Sa A,\Box\Theta
    }
\end{equation}
As is well know, cut elimination fails but as shown by Takano~\cite{Tak92} the calculus
%Takano~\cite{Tak92} showed that it 
has the analytic cut property.
%using a syntactic argument similar to ours for $\BiInt$. 
%
Cut-restriction provides a proof too. 
%As the proofs follows essentially the same steps as for $\BiInt$, we  
%\agata{check that the identified properties are satisfied, and show an example case.
%identify the core ideas.
%Let us discuss along the lines of the general discussion in the previous section why Takano's result holds. First, 

First notice that  $\SF$ admit principal cut reductions for all connectives, and axiom expansion. Also, the left and right rules of $\land$ and $\lor$ are invertible.
%just as in classical logic (or $\BiInt$). 
As the implication $A\imp B$ is classical, it can be considered as a derived connective and therefore removed from the signature. The role of the problematic connectives for cut-elimination ($\imp$
and $\coimp$ in $\BiInt$) is taken here by the modality $\Box$.

A boxed formula is principal in the antecedent by~$T$ (``left rule'') and in the succedent by~$5$ (``right rule'').
In the latter, the context consists of boxed formulas only, namely $\Box\Gamma$ in the antecedent and $\Box\Theta$ in the succedent. For every non-initial rule instance in $\SF$, appending arbitrary multisets of boxed formulas to the antecedent and succedent yields a new rule instance. 
%$(\Box\Gamma,\Box\Theta)$ and $(\Box\Theta,\Box\Gamma)$. 
It follows that $\Box$ is \textbf{right-compatible}. Once this is noted, essentially the same proof as for Theorem~\ref{thm:main} also works for $\SF$.
%
For illustration, we picture a simple case below.

%As all rules for classical connectives are locally analytic hp-invertible (see the Appendix), the only problematic cuts to handle are those on boxed formulas. Similarly as the cases for the implication and the co-implication in $\BiInt$, we trace the boxed cut formula $\Box A$ upwards until it is principal in the rule $T$ or $5$. This time the critical set of an inference of $5$ is defined to be $\Box\Gamma\cup\Box\Delta$. The cut on $\Box A$ can then be replaced by cuts on all critical formulas. We illustrate one simple case in which there is only one critical formula $\Box\gamma$:

%The rules for the $\Box$ modalities are not locally analytic hp-invertible. We therefore prove that they satisfies the conditions of Theorem~\ref{generic}.
%\begin{corollary}
%The calculus for $\SF$ in \cite{OhnMat57} has the analytic cut property.
%\end{corollary}


%Similarly as the cases for the implication and the co-implication in $\BiInt$, we trace the boxed cut formula $\Box A$ upwards until it is principal in the rule $T$ or $5$. This time the critical set of an inference of $5$ is defined to be $\Box\Gamma\cup\Box\Delta$. The cut on $\Box A$ can then be replaced by cuts on all critical formulas. We illustrate one simple case in which there is only one critical formula $\Box\gamma$:
%@{\hspace{1em}to\hspace{1em}}
\begin{center}
\begin{tabular}{c@{\hspace{1em}to\hspace{1em}}c}
\begin{footnotesize}
$
\infer[\cut]{\Gamma\Sa\Delta}
    {
    \infer*{\Gamma\Sa\Box A,\Delta}
        {
        \infer[5]{\Box D\Sa\Box A}
            {
            \Box D\Sa A
            }
        }
    &
    \infer*{\Gamma,\Box A\Sa \Delta}
        {
        \infer[T]{ \Sigma,\Box A\Sa \Pi}
            {
            \Sigma,A\Sa \Pi
            }
        }
    }
$
\end{footnotesize}
%\end{center}
&
%\AxiomC{to}
%\noLine
%\UnaryInfC{\phantom{A}}
%\noLine
%\UnaryInfC{\phantom{A}}
%\noLine
%\UnaryInfC{\phantom{A}}
%\noLine
%\UnaryInfC{\phantom{A}}
%\DisplayProof
%&
\begin{footnotesize}
$
\infer[cut]{\Gamma\Sa\Delta}
    {
    \infer*{\Gamma\Sa\Box D,\Delta}
        {
        \Box D\Sa\Box D
        }
    &
    \infer*{\Gamma,\Box D\Sa\Delta}
        {
        \infer[cut*]{ \Sigma,\Box D\Sa \Pi}
            {
            \Box D\Sa A
            &
            \Sigma,A\Sa \Pi
            }
        }
    }
$
\end{footnotesize}
\end{tabular}
%\vspace{-1cm}
\end{center}
%Again we can argue that if the cut on $\Box A$ was the uppermost non-analytic one, then either $\Box\gamma$ is a proper subformula of $\Box A$, or $\Box\gamma$ is a subformula of $\Gamma\cup\Delta$.

%It is crucial here that $\botpart{\delta}{\Box A}[\Sigma]$ and $\botpart{\epsilon}{\Box A}[\Sigma]$ are only well-defined derivations if $\Sigma$ consists solely of boxed formulas, as adding unboxed formulas to an inference of $5$ breaks soundness. In the case of the above transformation this is guaranteed since every critical formula comes from the context of an inference of $5$, and therefore must be boxed.



